Making View Update Strategies Programmable - Toward Controlling and Sharing Distributed Data -

Views are known mechanisms for controlling access of data and for sharing data of different schemas. Despite long and intensive research on views in both the database community and the programming language community, we are facing difficulties to use views in practice. The main reason is that we lack ways to directly describe view update strategies to deal with the inherent ambiguity of view updating. This paper aims to provide a new language-based approach to controlling and sharing distributed data based on views, and establish a software foundation for systematic construction of such data management systems. Our key observation is that a view should be defined through a view update strategy rather than a view definition. We show that Datalog can be used for specifying view update strategies whose unique view definition can be automatically derived, present a novel P2P-based programmable architecture for distributed data management where updatable views are fully utilized for controlling and sharing distributed data, and demonstrate its usefulness through the development of a privacy-preserving ride-sharing alliance system.

==> implementation1.tex <==
%!TEX root = main.tex
% \section{Implementation of Programmable Architecture}
% \label{sec:implementationArchitecture}
%
% This section will explain how to implement the programmable architecture using PostgreSQL.

\input{ImpleOverview}
%\input{Incrementalization}
%\input{ImplementationInPostgreSQL}


==> implementation2.tex <==
\section{An Application}
%: Privacy-Preserving Ride-Sharing Alliance System}
\label{sec:impRideSharing}
\begin{figure}[ttt]
  \centerline{\includegraphics[width=0.45\textwidth]{figure5-4_implementation.pdf}}
  \caption{A framework for Privacy-Preserving Ride-Sharing Alliance System}
  \label{fig:rideSharingSystem}
\end{figure}
We explain the implementation details of the privacy-preserving ride-sharing alliance system as described in Section \ref{sec:ridesharing}.
The system provides a data to book an appropriate taxi for a passenger.
Figure \ref{fig:rideSharingSystem} shows a framework for the system.
The mediator integrates data from multiple taxi companies that manage their own databases whose schemes are different each other.
%To achieve self-controllable data, we use {\em a view updating} provided by PostgreSQL.


% \begin{figure}
%   \centerline{\includegraphics[width=0.7\textwidth]{rideSharing.png}}
%   \caption{A Ride-Sharing System}
%   \label{fig:rideSharingSystem}
% \end{figure}

\subsection{Basic Parts}
To implement the framework of the system, we need to implement the basic parts (i.e., data controller, data integrator, and data connector in Section \ref{subsec:basicideas}).
In addition, we implement a function to analysis user requests.

\input{localschema}
\input{mediatedschema}
\input{dataconnecter}
\subsection{Data Analysis on Mediator}
\label{subsec:analysis}
\input{analysis}

%\subsubsection{Discussions}
%\input{implementationDiscussion}


==> implementationInPostgreSQL.tex <==
\subsection{Implementing BX in PostgreSQL}
\label{subsec:impBXinPosgreSQL}
%We show how to implement a bidirectional update propagation in PostgreSQL. 
In this subsection, we briefly describes an important implementation issue that 
how the BX can be systematically implemented in PostgreSQL. 
We use {\em triggers}, which can be used to define functions 
based on ECA(Event, Condition and Action)-rules. 
As a language for defining trigger functions,
a PostgreSQL-dialect of PL/SQL called PL/pgSQL
has enough expressive power to implement the update strategy.
As described above, there are two kinds of BX 
in the programmable architecture. One is established 
in the data controller, the other is established in the data
integrator. 
For each BX (a derived $get$ and a predefined $put$), bidirectional
update propagation can be realized by 
preparing two triggers, one is defined on views and the other is
defined on tables, which compose the views. 
Note that one may implement a bidirectional update propagation
by preparing two trigger functions, independently. However, in such 
implementations, the important property, the round-trip property shown in
the introduction, can not be guaranteed. 
Instead, we define two trigger functions satisfying the property 
by translating through the well-behaved BX (a $get$ and a $put$). 
Note also that we need to avoid falling in infinite loops by
pulling the triggers in both sides.  

% In integrated views, one trigger is defined over
% the mediator to propagate updates on the mediator into the controlled
% data, and the other trigger is defined on the controlled data to
% propagate updates on the controlled data into the mediator. 
% In the each local database, one trigger is defined over the controlled
% data to propagate updates on the controlled data into the local data,
% and the other trigger is defined on the local data to propagate
% updates on the local data into the controlled data. 

Since both the views of self-controllable data in the data controller
and integrated views in data integrator are materialized, both
an incremental version of view maintenance for 
$get$ and an incremental version of $put$ with respect to the updates are
needed to implement the updates propagation in trigger functions
to reflect both updates on sources and views efficiently.
So, the incremental version of view maintenance for $get$ with respect
to an update on a source specifies how to reflect an update to the
materialized view when the update is executed to source data.
Whereas, the incremental version of $put$ specifies
how to reflect an update to the source data
when the update is executed to a view.
In other words, for given a source database $S$, a view definition $get$
and an update $w$ on the source $S$, an incremental version of view
maintenance for $get$ with respect to $w$ denoted by $w'$
satisfies the following equation: 
\[
get(w(S)) = w' (get(S))
\]
Also, for given a materialized view $V$, an update strategy $put$ and an
update $u$ on the view $V$, an incremental version of $put$ with
respect to $u$ denoted by $u'$ satisfies the following equation:
\[
put(S, u(V)) = u'(V)
\]
Note that we can apply the existing work \cite{AKKN12} and
\cite{Horn17} to obtain an incremental view maintenance for $get$ and 
an incremental update strategy for $put$, respectively. 

Now, we show, for given a BX (a $get$ and a $put$), the whole steps to
implement two trigger functions, one is for a $get$ and the other is
for a $put$ by using the examples shown in Section~\ref{sec:RU-sharing}. 
%
For implementing a $get$, we use the following two steps:
\begin{enumerate}
\item[(g1)] Deriving an incremental version of view maintenance. \\
An incremental version of view maintenance for $get$ with respect to an update on
a source can be obtained based on a static analysis \cite{AKKN12}.  
For example, when the following insertion $w$ is
executed to \verb|vehicles| shown in Section~\ref{sec:RU-sharing}: 
\begin{verbatim}
  INSERT INTO vehicles
  VALUES (new_vid, new_loc, new_rid)
\end{verbatim}
the following $w'$ can be obtained from the view definition 
$get$ derived from the update strategy for \verb|peer1_public| shown in 
Section~\ref{sec:RU-sharing}: 
\begin{verbatim}
  INSERT INTO public_peer1
  SELECT new_vid, area, new_rid
  FROM   area_map
  WHERE  area_map.loc = new_loc
\end{verbatim}
\item[(g2)] Translating the incremental view maintenance into a trigger function.\\
  For example, the above incremental version of view maintenance can be translated
  into the following pseudo code in trigger function defined on
  \verb|vehicles|: 
\begin{verbatim}
  CREATE OR REPLACE FUNCTION
    vehicles()
  RETURNS trigger AS $$
    BEGIN
      IF TG_OP ='INSERT' THEN
        INSERT INTO public_peer1
        SELECT NEW.vid, area, NEW.rid
        FROM area_map
        WHERE area_map.loc=New.loc;
      ELSE ...
      END IF;
      RETURN NEW;
    END;
  $$ LANGUAGE plpgsql;
\end{verbatim}
The above trigger function works that when an event of insertion to
\verb|vehicles| is happened, the insertion of the incremental view
maintenance to \verb|public_peer1| is also executed. 
\end{enumerate}  

Similarly, for implementing a $put$, we use the following two steps:
\begin{enumerate}
\item[(p1)] Deriving an incremental version of an update strategy.\\
An incremental version of $put$ with respect to an update on a view can
be obtained based on a static analysis \cite{Horn17}. 
For example, when the following update $u$ is executed to
\verb|peer1_public|: 
\begin{verbatim}
  UPDATE peer1_public
  SET    request_id = new_id
  WHERE  viehicle_id = id
\end{verbatim}
the following $u'$ can be
obtained for a given update strategy shown in
Section~\ref{sec:RU-sharing}: 
\begin{verbatim}
  UPDATE vehicle
  SET    rid = new_rid
  WHERE  vid = id
\end{verbatim}
\item[(p2)] Translating the incremental $put$ into a trigger function.\\
  For example, the above incremental version of update strategy can be
  translated into the following
  pseudo code in trigger function is defined on \verb|peer1_public|:
\begin{verbatim}
  CREATE OR REPLACE FUNCTION
  update_peer1_public()
  RETURNS trigger AS $$
    BEGIN
      IF TG_OP = 'UPDATE' THEN
        UPDATE vehicle
        SET
          rid = NEW.request_id
        WHERE
          vid = NEW.vehicle_id;
      ELSE ...
      END IF;
      RETURN NEW;
    END;
  $$ LANGUAGE plpgsql;
\end{verbatim}
The above trigger function works that when an event of update on 
\verb|public_peer1| is happened, the update of the incremental $put$ 
on \verb|vehicles| is also executed. 
\end{enumerate}  


==> implementation_ridesharing_p2p.tex <==
\subsection{P2P Architecture for Ride-Sharing Alliance}
%\todo{Sasaki will shorten this section (0.2 page?)}
%We explain the implementation details of the privacy-preserving ride-sharing alliance system.
%The system provides a data to book an appropriate taxi for a passenger.
Ride-sharing companies freely join in and leave from the ride-sharing system as peers.
The system is composed of two kinds of peers; provider and mediator.
When the companies join the system, they become providers which manage their own databases and provide their data to the mediator.
The mediator integrates data from multiple providers and analyses passengers' requests.

%Each taxi company maintains their own database.
%To simplify the discussion, we assume two taxi companies use different schema as shown in Section \ref{sec:language}.
%In each database, there are multiple tables and one materialized view.% ({\tt peer$i$\_public}).
%data control
Each provider sets {\tt peer$i$\_public} as the Dejima table, and each Dejima table synchronizes with the Dejima tables at the mediator.
%{\tt peer$i$\_public} is used to provide information from each company to the mediator.
These Dejima tables conceal the private data such as the precise locations of the vehicles.
The mediator integrates the disclosed data as an integrated view.
It uses the integrated view for analyzing the benefits of providers based on the passengers' requests.
%In our implementation, the mediator and each provider are connected by FDW, and thus each {\tt peer$i\_$public} on the mediator is defined as a foreign table.

Each database of the provider is {\em self-controllable} since it is managed only by itself.
As an exception, disclosed data can be updated from the mediator only through the Dejima table.
The mediator updates the data to book vehicles for passengers.
The update may not be allowed because the vehicles may be already booked by other passengers.
This function is provided by the bidirectional view update.
%For handling this case, each peer sends back error messages.
The implementation is available online \cite{Proto}.

%, and if the mediator receives the messages, it analyzes the passengers' requests again.
%To this end, we use  triggers which are executed at each provider.

%mediator


%Then, it shows a list of $K$ vehicles with the highest benefits to passengers.

%The integrated view i, and it provides data in a common schema for the analysis.
%{\tt all$\_$vehicles} is created  as a virtual view on the mediator by the query descried in Section \ref{sec:RU-integration}.
%Since the mediator updates {\tt all$\_$vehicles} for booking taxis, the update is propagated to the database at each peer.
%We have two triggers on mediator for updating the integrated view and  {\tt peer$i$$\_$public} view of each provider $i$.
%For instance, the following describes the triggler for updating {\tt all$\_$vehicles} from provider 1.
%connector
%The mediator and each provider are connected by FDW, and thus each {\tt peer$i$$\_$public} on the mediator is defined as a foreign table.
%The databases on the providers may not allow updating because a vehicle that is tried to be booked may be already booked by other passengers.
%For handling this case, each peer sends back error messages, and if the mediator receives the messages, it analyzes the passengers' requests again.
%analysis
%The mediator receives the passengers' requests and analyzes the benefits of providers based on the requests and the integrated view.
%time of the request and the locations of the start point, destination, and vehicles.


%We open the code for ride-sharing alliance system\footnote{https://github.com/dangtv/RelationalViewUpdate}.


==> ridesharing.tex <==
\subsection{Implementation: Ride-sharing Alliance System}
\todo{Sasaki will shorten this section (0.4 page?) depending on contents in Section 2?}
We explain the implementation details of the privacy-preserving ride-sharing alliance system.
The system provides a data to book an appropriate taxi for a passenger.
It composes of two kinds of peers; provider and mediator.
The provider provides their own data.
The mediator integrates data from multiple taxi companies that manage their own databases whose schemes are different each other.

Each taxi company maintains their own database.
To simplify the discussion, we assume two taxi companies use different schema as shown in Section \ref{sec:language}. 
In each database, there are multiple tables and one materialized view.% ({\tt peer$i$\_public}). 

%data control
{\tt peer$i$\_public} is used to provide information from each company to the mediator. 
This view conceals the private information such as the precise locations of the vehicles.  

Each database of a taxi company is {\em self-controlable} since it is managed only by the taxi company while {\tt peer$i$\_public} is used for exporting data to the mediator.
Each table (such as {\tt vehicles} table at provider 1) can be updated from outside only through the update of {\tt peer$i$\_public}.
To this end, we use  triggers provided described in Section \ref{subsec:impBXinPosgreSQL}.
This trigger is executed at each provider (the lower part of Figure \ref{fig:rideSharingSystem}).

%mediator
The mediator integrates the disclosed information on each peer as an integrated view {\tt all$\_$vehicles}, and it provides data in a common schema for the analysis.
{\tt all$\_$vehicles} is created  as a virtual view on the mediator by the query descried in Section \ref{sec:RU-integration}.
Since the mediator updates {\tt all$\_$vehicles} for booking taxis, the update is propagated to the database at each peer.
We have two triggers on mediator for updating the {\tt all$\_$vehicles} view and  {\tt peer$i$$\_$public} view of each provider $i$.
For instance, the following describes the triggler for updating {\tt all$\_$vehicles} from provider 1.

%connector
The mediator and each provider are connected by FDW, and thus each {\tt peer$i$$\_$public} on the mediator is defined as a foreign table.
The databases on the providers may not allow updating because a vehicle that is tried to be booked may be already booked by other passengers.
For handling this case, each peer sends back error messages, and if the mediator receives the messages, it analyzes the passengers' requests again.

%analysis
The system analyzes the passenger request, and then shows a list of taxis to passengers.
We describe how the mediator analyzes data on the integrated view. 
The system analyzes the benefits of taxi companies based on the time of the request and the locations of the start point, destination, and vehicles. 
For example, it lists $K$ taxis with the highest benefits.

We open the code for ride-sharing alliance system\footnote{https://github.com/hiroyukikato/DataIntegration}.
